Multi-Source and Test-Time Domain Adaptation on Multivariate Signals using Spatio-Temporal Monge Alignment

Machine learning applications on signals such as computer vision or biomedical data often face significant challenges due to the variability that exists across hardware devices or session recordings. This variability poses a Domain Adaptation (DA) problem, as training and testing data distributions often differ. In this work, we propose Spatio-Temporal Monge Alignment (STMA) to mitigate these variabilities. This Optimal Transport (OT) based method adapts the cross-power spectrum density (cross-PSD) of multivariate signals by mapping them to the Wasserstein barycenter of source domains (multi-source DA). Predictions for new domains can be done with a filtering without the need for retraining a model with source data (test-time DA). We also study and discuss two special cases of the method, Temporal Monge Alignment (TMA) and Spatial Monge Alignment (SMA). Non-asymptotic concentration bounds are derived for the mappings estimation, which reveals a bias-plus-variance error structure with a variance decay rate of $\mathcal{O}(n_\ell^{-1/2})$ with $n_\ell$ the signal length. This theoretical guarantee demonstrates the efficiency of the proposed computational schema. Numerical experiments on multivariate biosignals and image data show that STMA leads to significant and consistent performance gains between datasets acquired with very different settings. Notably, STMA is a pre-processing step complementary to state-of-the-art deep learning methods.

==> old_stuff/old_proof.tex <==
\begin{theorem}[Concentration bound]
    \label{the:concentration_temp}
    \sloppy Let $\bX = [\bx_1, \dots, \bx_C]^\trans \in \bbR^{C\times T}$ be a realization of $\vect(\bX) \sim \cN(\mathbf{0}, \bSigma)$.
    For $k \in \intset{K}$, let $\bX_k \in \bbR^{C\times T}$ be a realization of $\vect(\bX_k) \sim \cN(\mathbf{0}, \bSigma_{k})$.
    Let us assume that $\bSigma$ and $\bSigma_k$ respect the Assumption~\ref{assu:temp}, \ie $\bSigma = \bF \diag(\bq_{1}, \dots, \bq_{C}) \bF^*$ and $\bSigma_k = \bF \diag(\bq_{1}^{k}, \dots, \bq_{C}^{k}) \bF^*$.
    For every $i \in \intset{C}$ and by denoting
    $\diag(\bp_i) = g_F(\diag(\bq_i))$,
    $\diag(\overline\bp_i) = g_F(\diag(\overline\bq_i))$, $\diag(\bp_{i}^{k}) = g_F(\diag(\bq_{i}^{k}))$,
    $\bh_i = \frac{1}{\sqrt{F}} \bS_F\bF_F^* \left({\overline{\bp}_i}^{\odot\frac{1}{2}}\odot {\bp_i}^{\odot-\frac{1}{2}} \right)$,
    there exists $c, C > 0$ independent from $T$ and $F$ such that with probability greater than $1-\delta$, we have
    \begin{align*}
        &\frac{\Vert \widehat\bh_i - \bh_i \Vert_\infty}{\Vert \widehat{\bp}_i^{\odot-\frac{1}{2}} \Vert_\infty} \leq \frac{1}{K} \sum_{k=1}^K \Vert\bb_{i}^{k}\Vert_\infty \Vert{\bp_{i}^{k}}^{\odot-\frac{1}{2}}\Vert_\infty + \Vert\overline{\bp}_i^{\odot\frac{1}{2}}\Vert_\infty  \Vert\bb_i\Vert_\infty \Vert\bp_i^{\odot-1}\Vert_\infty +\\
        &\quad C^2\sqrt{\frac{F}{T}} \left[ \frac{1}{K} \sum_{k=1}^K \Vert\bq_{i}^{k}\Vert_\infty \Vert{\bp_{i}^{k}}^{\odot-\frac{1}{2}}\Vert_\infty + \Vert\overline{\bp}_i^{\odot\frac{1}{2}}\Vert_\infty \Vert\bq_i\Vert_\infty \Vert\bp_i^{\odot-1}\Vert_\infty \right] \max\left(\sqrt{\frac{\log\left(\frac{2}{\delta}\right)}{c}},  \sqrt{\frac{F}{T}}\frac{\log\left(\frac{2}{\delta}\right)}{c}\right).
    \end{align*}
    where
    \begin{equation*}
        \displaystyle (\bb_i)_j = \frac{F}{T}\sum_{\substack{l=1\\ l \notin \{1, \frac{T}{F} + 1, \dots, \\ \frac{(F-1)T}{F} +1 \} }}^T (\bq_i)_l \bbf_{l,T}^* \left(\bI_\frac{T}{F} \otimes \bbf_{j,F}\bbf_{j,F}^*\right) \bbf_{l,T},
    \end{equation*}
    $\bb_{i}^{k}$ is obtained by replacing $\bq_i$ by $\bq_{i}^{k}$ and $\bbf_{l,Q}$ is the $l^\text{th}$ column of $\bF_Q$.
\end{theorem}

\begin{definition}[Barlett estimator]
    \label{def:welch}
    Let $\bX = [\bx_1, \dots, \bx_C]^\trans \in \bbR^{C\times T}$ be a realization of $\vect(\bX) \sim \cN(\mathbf{0}, \bSigma)$ and following the Assumption~\ref{assu:temp}, \ie $\bSigma = \bF\diag(\bq_1, \dots, \bq_C)\bF^*$, the Barlett estimator $\widehat{\bp}_i \in \bbR^F$ of $\diag(\bp_i) = g_F(\diag(\bq_i))$ is
    \begin{equation*}
        \widehat{\bp}_i = \frac{1}{\floor{T/F}} \sum_{t=1}^{\floor{T/F}} \left\vert \bF_F \widetilde\bx_{i, (t-1)F+1} \right\vert^{\odot 2}
    \end{equation*}
    where $\widetilde\bx_{i,t} = ((\bx_i)_{t}, \dots, (\bx_i)_{t+F})^\trans \in \bbR^F$.
    % \begin{equation*}
    %     \widehat{\bp}_F = \frac{\sqrt{F}}{T-F+1} \bF_F \sum_{t=1}^{T-F+1} (\bx)_t \widetilde\bx_t
    % \end{equation*}
    % where $\widetilde\bx_t = [\bx_{[t:t+\ceil{F/2}]}^\trans, \bx_{[t+\ceil{F/2}:t+1]}^\trans]^\trans\in \bbR^F$.
    % \begin{equation*}
    %     \begin{aligned}
    %         \bbE\left[\widehat{\bp}_F\right] &= \frac{\sqrt{F}}{T-F+1} \bF_F \sum_{t=1}^{T-F+1} \bbE\left[(\bx)_t \widetilde\bx_t\right] \\
    %         & = \frac{\sqrt{F}}{T-F+1} \bF_F \sum_{t=1}^{T-F+1} \bh_F \\
    %         & = \sqrt{F} \bF_F \bh_F = \bp_F.
    %     \end{aligned}
    % \end{equation*}
\end{definition}
% From Assumption~\ref{assu:temp}, the signals are spatially decorrelated and from Proposition~\ref{prop:temp_map} the $F$-Monge mapping is a convolution per sensor and performed with $\bh_i$.
For every $\bx \in \bbR^F$, and since $\bF_F$ is unitary, we have
\begin{align*}
    \Vert \bF_F \bx \Vert_\infty \geq \frac{1}{\sqrt{F}} \Vert \bF_F \bx \Vert_2 = \frac{1}{\sqrt{F}} \Vert \bx \Vert_2\geq \frac{1}{\sqrt{F}} \Vert \bx \Vert_\infty.
\end{align*}
Thus, for every $i \in \intset{C}$, we have
\begin{align*}
    \Vert \widehat\bh_i - \bh_i \Vert_\infty &\leq \sqrt{F} \left\Vert \bF_F \left(\widehat\bh_i - \bh_i\right)\right\Vert_\infty \\
    &= \left\Vert \widehat{\overline\bp}_i^{\odot\frac{1}{2}} \odot \widehat{\bp}_i^{\odot-\frac{1}{2}} - \overline\bp_i^{\odot\frac{1}{2}} \odot \bp_i^{\odot-\frac{1}{2}} \right\Vert_\infty.
\end{align*}
Using the triangle inequality and the sub-multiplicativity of the $\infty$-norm, we get that
\begin{align*}
    \Vert \widehat\bh_i - \bh_i \Vert_\infty &\leq \Vert \widehat{\overline\bp}_i^{\odot\frac{1}{2}} \odot \widehat{\bp}_i^{\odot-\frac{1}{2}} - \overline\bp_i^{\odot\frac{1}{2}} \odot \bp_i^{\odot-\frac{1}{2}} \Vert_\infty \\
    &= \Vert \widehat{\overline\bp}_i^{\odot\frac{1}{2}} \odot \widehat{\bp}_i^{\odot-\frac{1}{2}} - \overline\bp_i^{\odot\frac{1}{2}} \odot \widehat{\bp}_i^{\odot-\frac{1}{2}} + \overline\bp_i^{\odot\frac{1}{2}} \odot \widehat{\bp}_i^{\odot-\frac{1}{2}} - \overline\bp_i^{\odot\frac{1}{2}} \odot \bp_i^{\odot-\frac{1}{2}} \Vert_\infty \\
    &\leq \Vert \widehat{\overline\bp}_i^{\odot\frac{1}{2}} \odot \widehat{\bp}_i^{\odot-\frac{1}{2}} - \overline\bp_i^{\odot\frac{1}{2}} \odot \widehat{\bp}_i^{\odot-\frac{1}{2}} \Vert_\infty + \Vert \overline\bp_i^{\odot\frac{1}{2}} \odot \widehat{\bp}_i^{\odot-\frac{1}{2}} - \overline\bp_i^{\odot\frac{1}{2}} \odot \bp_i^{\odot-\frac{1}{2}} \Vert_\infty \\
    &\leq \Vert \widehat{\bp}_i^{\odot-\frac{1}{2}} \Vert_\infty \Vert \widehat{\overline\bp}_i^{\odot\frac{1}{2}} - \overline\bp_i^{\odot\frac{1}{2}} \Vert_\infty + \Vert \overline\bp_i^{\odot\frac{1}{2}} \Vert_\infty \Vert \widehat{\bp}_i^{\odot-\frac{1}{2}} - \bp_i^{\odot-\frac{1}{2}} \Vert_\infty \;.
\end{align*}
The barycenter is $\overline{\bp}_i^{\odot\frac{1}{2}} = \frac{1}{K} \sum_{k=1}^K \bp_{i, k}^{\odot\frac{1}{2}}$.
Thus, we get an upper-bound of the barycenter estimation error in terms of source PSD estimation errors, 
\begin{align*}
    \Vert \widehat{\overline\bp}_i^{\odot\frac{1}{2}} - \overline\bp_i^{\odot\frac{1}{2}} \Vert_\infty \leq \frac{1}{K} \sum_{k=1}^K \Vert \widehat{\bp}_{i,k}^{\odot\frac{1}{2}} - \bp_{i,k}^{\odot\frac{1}{2}} \Vert_\infty \;.
\end{align*}
Then, we upper-bound the source PSD estimation error
\begin{align*}
    \Vert \widehat{\bp}_{i,k}^{\odot\frac{1}{2}} - \bp_{i,k}^{\odot\frac{1}{2}} \Vert_\infty &= \max_{j \in \intset{F}}\left\vert \left({\widehat\bp}_{i,k}\right)_j^{\frac{1}{2}} -  \left({\bp}_{i,k}\right)_j^{\frac{1}{2}} \right\vert \\
    &= \max_{j \in \intset{F}}\left\vert \frac{\left(\left( {\widehat\bp}_{i,k} \right)_j^{\frac{1}{2}} - \left( {\bp}_{i,k} \right)_j^{\frac{1}{2}} \right)\left(\left( {\widehat\bp}_{i,k} \right)_j^{\frac{1}{2}} +  \left( {\bp}_{i,k} \right)_j^{\frac{1}{2}} \right)}{\left( {\widehat\bp}_{i,k} \right)_j^{\frac{1}{2}} +  \left( {\bp}_{i,k} \right)_j^{\frac{1}{2}}}\right\vert\\
    &= \max_{j \in \intset{F}}\left\vert \frac{\left( {\widehat\bp}_{i,k} \right)_j -  \left( {\bp}_{i,k} \right)_j}{\left( {\widehat\bp}_{i,k} \right)_j^{\frac{1}{2}} +  \left( {\bp}_{i,k} \right)_j^{\frac{1}{2}}}\right\vert \\
    &\leq \max_{j \in \intset{F}}\left\vert \frac{\left( {\widehat\bp}_{i,k} \right)_j -  \left( {\bp}_{i,k} \right)_j}{\left( {\bp}_{i,k} \right)_j^{\frac{1}{2}}}\right\vert.
\end{align*}
Hence, the barycenter estimation error is upper bounded by
\begin{equation}
    \label{eq:mean_ineq}
    \Vert \widehat{\overline\bp}_i^{\odot\frac{1}{2}} - \overline\bp_i^{\odot\frac{1}{2}} \Vert_\infty \leq \frac{1}{K} \sum_{k=1}^K \max_{j \in \intset{F}}\left\vert \frac{\left( {\widehat\bp}_{i,k} \right)_j -  \left( {\bp}_{i,k} \right)_j}{ \left( {\bp}_{i,k} \right)_j^{\frac{1}{2}}}\right\vert.
\end{equation}
We denote $\bbf_{j,F} \in \bbC^F$ the $j^\text{th}$ column of $\bF_F$,
$\bx_{i,k} \in \bbR^T$ the time series of the $i^\text{th}$ sensor from the $k^\text{th}$ domain,
$\bz_{i,k} = \bSigma_{i,k}^{-\frac{1}{2}} \bx_{i,k}$ the whiten time series and 
$\widetilde\bx_{i,k,t} = \left((\bx_{i,k})_t, \dots, (\bx_{i,k})_{t+F-1}\right)^\trans \in \bbR^F$.
From Definition~\ref{def:welch}, we have
\begin{align*}
    (\widehat\bp_{i,k})_j &= \frac{F}{T} \sum_{t=1}^{T/F} \bbf_{j,F}^* \widetilde\bx_{i,k,(t-1)F+1} \widetilde\bx_{i,k,(t-1)F+1}^\trans \bbf_{j,F} \\
     &= \frac{F}{T} \bx_{i,k}^\trans \left(\bI_{\frac{T}{F}} \otimes \bbf_{j,F}\bbf_{j,F}^*\right) \bx_{i,k}\\
     &= \frac{F}{T} \bz_{i,k}^\trans \bSigma_{i,k}^\frac{1}{2} \left(\bI_{\frac{T}{F}} \otimes \bbf_{j,F}\bbf_{j,F}^*\right)\bSigma_{i,k}^\frac{1}{2} \bz_{i,k} \\
     &= \bz_{i,k}^\trans \bQ_{i,k,j} \bz_{i,k}
\end{align*}
where $\bQ_{i,k,j} = \frac{F}{T} \bSigma_{i,k}^\frac{1}{2} \left(\bI_{\frac{T}{F}} \otimes \bbf_{j,F}\bbf_{j,F}^*\right)\bSigma_{i,k}^\frac{1}{2} \in \mathbb{R}^{T \times T}$.
\begin{align*}
    \mathbb{E}\left[ (\widehat\bp_{i,k})_j \right] &= \mathbb{E}\left[ \bz_{i,k}^\trans \bQ_{i,k,j} \bz_{i,k} \right] \\
    &= \frac{F}{T} \Tr\left(\bSigma_{i,k}^\frac{1}{2} \left(\bI_{\frac{T}{F}} \otimes \bbf_{j,F}\bbf_{j,F}^*\right)\bSigma_{i,k}^\frac{1}{2}\right) \\
    &= \frac{F}{T} \sum_{l=1}^T (\bq_{i,k})_l \bbf_{l,T}^* \left(\bI_{\frac{T}{F}} \otimes \bbf_{j,F}\bbf_{j,F}^*\right) \bbf_{l,T} \;.
\end{align*}
It should be noted that
\begin{equation*}
    \sum_{l=1}^T \bbf_{l,T}^* \left(\bI_{\frac{T}{F}} \otimes \bbf_{j,F}\bbf_{j,F}^*\right) \bbf_{l,T} = \Tr\left(\bI_{\frac{T}{F}} \otimes \bbf_{j,F}\bbf_{j,F}^*\right) = \frac{T}{F},
\end{equation*}
and 
\begin{equation*}
    \bbf_{l,T}^* \left(\bI_{\frac{T}{F}} \otimes \bbf_{j,F}\bbf_{j,F}^*\right) \bbf_{l,T} =
    \begin{cases}
        1 \quad \text{if} \,\, l = \frac{(j-1)T}{F} + 1, \\
        0 \quad \text{if} \,\, l=\frac{(m-1)T}{F} + 1 \,\, \text{with} \, m \neq j \;.
    \end{cases}
\end{equation*}
Hence, we get that
\begin{equation*}
    \bbE\left[ (\widehat\bp_{i,k})_j \right] = (\bq_{i,k})_{\frac{(j-1)T}{F} + 1} + (\bb_{i,k})_j = (\bp_{i,k})_{j} + (\bb_{i,k})_j
\end{equation*}
where
\begin{equation*}
    (\bb_{i,k})_j = \frac{F}{T}\sum_{\substack{l=1\\ l \notin \{1, \frac{T}{F} + 1, \dots, \\ \frac{(F-1)T}{F} +1 \} }}^T (\bq_{i,k})_l \bbf_{l,T}^* \left(\bI_\frac{T}{F} \otimes \bbf_{j,F}\bbf_{j,F}^*\right) \bbf_{l,T}.
\end{equation*}
For $F=T$, we get that $\bb_{i,k}=\mathbf{0}$.
For $F=1$, we have
\begin{equation*}
    (\bb_{i,k})_j = \frac{1}{T}\sum_{\substack{l=1\\ l \neq \frac{(j-1)T}{F} +1}}^T (\bq_{i,k})_l \;.
\end{equation*}
This was expected since for $F=1$, 
\begin{equation*}
    \bbE\left[\widehat\bp_{i,k}\right] = \bbE\left[\frac{1}{T}\sum_{t=1}^T (\bx_{i,k})_t^2\right] = \frac{1}{T} \bbE\left[\Tr\left(\bx_{i,k}\bx_{i,k}^\trans \right)\right] =\frac{1}{T} \Tr(\bSigma_{i,k}) = \frac{1}{T} \sum_{t=1}^T (\bq_{i,k})_t.
\end{equation*}
We now leverage the Hanson-Wright inequality from~\cite{rudelson_hanson-wright_2013} to upper-bound the estimation error of $(\widehat\bp_{i,k})_j$,
\begin{equation*}
    \bbP\left(|(\widehat\bp_{i,k})_j - (\bp_{i,k})_j - (\bb_{i,k})_j| \leq t \right) \geq
    1 - 2 \exp\left( -c \min\left(\frac{t^2}{C^4 \Vert \bQ_{i,k,j} \Vert_F^2}, \frac{t}{C^2 \Vert \bQ_{i,k,j} \Vert} \right) \right).
\end{equation*}
Furthermore, if we set a $1-\delta$ probability threshold, \ie
\begin{equation*}
    1 - \delta =   1 - 2 \exp\left( -c \min\left(\frac{t^2}{C^4 \Vert \bQ_{i,k,j} \Vert_F^2}, \frac{t}{C^2 \Vert \bQ_{i,k,j} \Vert} \right) \right)
\end{equation*}
then, equivalently, we get
\begin{equation*}
     \frac{t}{C^2} \min\left(\frac{t}{C^2 \Vert \bQ_{i,k,j} \Vert_F^2}, \frac{1}{\Vert \bQ_{i,k,j} \Vert} \right) = \frac{\log\left(\frac{2}{\delta}\right)}{c}.
\end{equation*}
If $t < C^2 \frac{\Vert \bQ_{i,k,j} \Vert_F^2}{\Vert \bQ_{i,k,j} \Vert}$ then $t = C^2 \Vert \bQ_{i,k,j} \Vert_F \sqrt{\frac{\log\left(\frac{2}{\delta}\right)}{c}}$  otherwise $t = C^2 \frac{\Vert \bQ_{i,k,j} \Vert\log\left(\frac{2}{\delta}\right)}{c}$.
Thus, with probability greater than $1-\delta$, we have
\begin{equation*}
    |(\widehat{\bp}_{i,k})_j - (\bp_{i,k})_j - (\bb_{i,k})_j| \leq C^2 \max\left(\Vert \bQ_{i,k,j} \Vert_F \sqrt{\frac{\log\left(\frac{2}{\delta}\right)}{c}},  \Vert \bQ_{i,k,j} \Vert \frac{\log\left(\frac{2}{\delta}\right)}{c} \right).
\end{equation*}
It remains to upper-bound $\Vert \bQ_{i,k,j} \Vert_F$ and $\Vert \bQ_{i,k,j} \Vert$.
We begin with the latter,
\begin{align*}
   \Vert \bQ_{i,k,j} \Vert &= \frac{F}{T} \left\Vert \bSigma_{i,k}^\frac{1}{2} \left(\bI_\frac{T}{F} \otimes \bbf_{j,F}\bbf_{j,F}^*\right)\bSigma_{i,k}^\frac{1}{2} \right\Vert \\
   &\leq \frac{F}{T} \left\Vert \bq_{i,k} \right\Vert_\infty \left\Vert \bI_\frac{T}{F} \otimes \bbf_{j,F}\bbf_{j,F}^*\right\Vert \\
   &= \frac{F}{T} \left\Vert \bq_{i,k} \right\Vert_\infty \;.
\end{align*}
Since $\text{rank}\left(\bSigma_{i,k}^\frac{1}{2} \left(\bI_\frac{T}{F} \otimes \bbf_{j,F}\bbf_{j,F}^*\right)\bSigma_{i,k}^\frac{1}{2}\right) = \frac{T}{F}$, we get the following upper-bound of $\Vert \bQ_{i,k,j} \Vert_F$,
\begin{align*}
   \Vert \bQ_{i,k,j} \Vert_F &= \frac{F}{T} \left\Vert \bSigma_{i,k}^\frac{1}{2} \left(\bI_\frac{T}{F} \otimes \bbf_{j,F}\bbf_{j,F}^*\right)\bSigma_{i,k}^\frac{1}{2} \right\Vert_F \\
   & \leq \frac{F}{T} \sqrt{\frac{T}{F}} \left\Vert \bSigma_{i,k}^\frac{1}{2} \left(\bI_\frac{T}{F} \otimes \bbf_{j,F}\bbf_{j,F}^*\right)\bSigma_{i,k}^\frac{1}{2} \right\Vert \\
   & \leq \sqrt{\frac{F}{T}} \left\Vert \bq_{i,k} \right\Vert_\infty.
\end{align*}
Thus, with probability greater than $1-\delta$, we get
\begin{equation}
    \label{PSD_est_upper}
    \frac{|(\widehat{\bp}_{i,k})_j - (\bp_{i,k})_j - (\bb_{i,k})_j|}{(\bp_{i,k})_j^\frac{1}{2}} \leq\\
    C^2 \sqrt{\frac{F}{T}}\frac{\left\Vert \bq_{i,k} \right\Vert_\infty}{(\bp_{i,k})_j^\frac{1}{2}}\max\left(\sqrt{\frac{\log\left(\frac{2}{\delta}\right)}{c}},  \sqrt{\frac{F}{T}}\frac{\log\left(\frac{2}{\delta}\right)}{c}\right).
\end{equation}
We now tackle~\autoref{eq:mean_ineq}, \ie the estimation error of the barycenter
\begin{align*}
    &\max_{j \in \intset{F}}\left\vert \frac{\left( \widehat{\bp}_{i,k} \right)_j -  \left( {\bp}_{i,k} \right)_j}{ \left( {\bp}_{i,k} \right)_j^{\frac{1}{2}}}\right\vert =  \max_{j \in \intset{F}}\left\vert \frac{\left( \widehat{\bp}_{i,k} \right)_j -  \left( {\bp}_{i,k} \right)_j - (\bb_{i,k})_j + (\bb_{i,k})_j}{ \left( {\bp}_{i,k} \right)_j^{\frac{1}{2}}}\right\vert\\
    &\leq  \max_{j \in \intset{F}}\left\vert \frac{(\bb_{i,k})_j}{ \left( {\bp}_{i,k} \right)_j^{\frac{1}{2}}}\right\vert +  \max_{j \in \intset{F}}\left\vert \frac{\left( \widehat{\bp}_{i,k} \right)_j -  \left( {\bp}_{i,k} \right)_j - (\bb_{i,k})_j}{ \left( {\bp}_{i,k} \right)_j^{\frac{1}{2}}}\right\vert \\
    &\leq  \Vert\bb_{i,k}\Vert_\infty \Vert\bp_{i,k}^{\odot-\frac{1}{2}}\Vert_\infty +  \max_{j \in \intset{F}}\left\vert \frac{\left( \widehat{\bp}_{i,k} \right)_j -  \left( {\bp}_{i,k} \right)_j - (\bb_{i,k})_j}{ \left( {\bp}_{i,k} \right)_j^{\frac{1}{2}}}\right\vert.
\end{align*}
Furthermore, using~\eqref{PSD_est_upper}, we have
\begin{equation*}
    \max_{j \in \intset{F}}\left\vert \frac{\left( \widehat{\bp}_{i,k} \right)_j - \left( {\bp}_{i,k} \right)_j - (\bb_{i,k})_j}{ \left( {\bp}_{i,k} \right)_j^{\frac{1}{2}}}\right\vert \leq C^2\sqrt{\frac{F}{T}} \Vert\bq_{i,k}\Vert_\infty \Vert\bp_{i,k}^{\odot-\frac{1}{2}} \Vert_\infty \max\left(\sqrt{\frac{\log\left(\frac{2}{\delta}\right)}{c}}, \sqrt{\frac{F}{T}}\frac{\log\left(\frac{2}{\delta}\right)}{c}\right).
\end{equation*}
From~\autoref{eq:mean_ineq}, we get the following upper-bound on the barycenter estimation error
\begin{align*}
    &\Vert \widehat{\overline\bp}_i^{\odot\frac{1}{2}} - \overline\bp_i^{\odot\frac{1}{2}} \Vert_\infty \leq \frac{1}{K} \sum_{k=1}^K \max_{j \in \intset{F}}\left\vert \frac{\left( \widehat{\bp}_{i,k} \right)_j -  \left( {\bp}_{i,k} \right)_j}{ \left( {\bp}_{i,k} \right)_j^{\frac{1}{2}}}\right\vert\\
    &\leq \frac{1}{K} \sum_{k=1}^K \Vert \bb_{i,k} \Vert_\infty \Vert\bp_{i,k}^{\odot-\frac{1}{2}}\Vert_\infty + C^2\sqrt{\frac{F}{T}} \left[ \frac{1}{K} \sum_{k=1}^K \Vert\bq_{i,k}\Vert_\infty \Vert\bp_{i,k}^{\odot-\frac{1}{2}}\Vert_\infty \right] \max\left(\sqrt{\frac{\log\left(\frac{2}{\delta}\right)}{c}},  \sqrt{\frac{F}{T}}\frac{\log\left(\frac{2}{\delta}\right)}{c}\right).
\end{align*}
We treat the estimation error of the target PSD,
\begin{align*}
   \Vert \widehat{\bp}_i^{\odot-\frac{1}{2}} - \bp_i^{\odot-\frac{1}{2}} \Vert_\infty &= \max_{j\in \intset{F}} \left\vert \frac{1}{(\widehat{\bp}_i)_j^\frac{1}{2}} - \frac{1}{(\bp_i)_j^\frac{1}{2}} \right\vert \\
   &= \max_{j\in \intset{F}} \left\vert \frac{(\widehat{\bp}_i)_j^\frac{1}{2} - (\bp_i)_j^\frac{1}{2}}{(\widehat{\bp}_i)_j^\frac{1}{2} (\bp_i)_j^\frac{1}{2}} \right\vert \\
   & \leq \Vert \widehat{\bp}_i^{\odot-\frac{1}{2}} \odot \bp_i^{\odot-\frac{1}{2}} \Vert_\infty \max_{j\in \intset{F}} \left\vert(\widehat{\bp}_i)_j^\frac{1}{2} - (\bp_i)_j^\frac{1}{2} \right\vert \\
   &\leq \Vert \widehat{\bp}_i^{\odot-\frac{1}{2}} \odot \bp_i^{\odot-\frac{1}{2}} \Vert_\infty \max_{j \in \intset{F}}\left\vert \frac{\left(\widehat{\bp}_i\right)_j -  \left(\bp_i\right)_j}{\left(\bp_i\right)_j^{\frac{1}{2}}}\right\vert.
\end{align*}
Thus, with probability greater than $1-\delta$, we get
\begin{equation*}
   \frac{\Vert \widehat{\bp}_i^{\odot-\frac{1}{2}} - \bp_i^{\odot-\frac{1}{2}} \Vert_\infty}{\Vert \widehat{\bp}_i^{\odot-\frac{1}{2}} \Vert_\infty} \leq
   \Vert \bb_i \Vert_\infty \Vert\bp_i^{\odot-1}\Vert_\infty  +
   C^2 \sqrt{\frac{F}{T}} \Vert\bq_i\Vert_\infty \Vert\bp_i^{\odot-1}\Vert_\infty \max\left(\sqrt{\frac{\log\left(\frac{2}{\delta}\right)}{c}},  \sqrt{\frac{F}{T}}\frac{\log\left(\frac{2}{\delta}\right)}{c}\right).
\end{equation*}
Combining everything, we get 
\begin{align*}
    &\frac{\Vert \widehat\bh_i - \bh_i \Vert_\infty}{\Vert \widehat{\bp}_i^{\odot-\frac{1}{2}} \Vert_\infty} \leq \Vert \widehat{\overline\bp}_i^{\odot\frac{1}{2}} -\overline\bp_i^{\odot\frac{1}{2}} \Vert_\infty + \Vert \overline\bp_i^{\odot\frac{1}{2}} \Vert_\infty \frac{\Vert \widehat{\bp}_i^{\odot-\frac{1}{2}} - \bp_i^{\odot-\frac{1}{2}} \Vert_\infty}{\Vert \widehat{\bp}_i^{\odot-\frac{1}{2}} \Vert_\infty} \\
    &\leq \frac{1}{K} \sum_{k=1}^K \Vert\bb_{i,k}\Vert_\infty \Vert\bp_{i,k}^{\odot-\frac{1}{2}}\Vert_\infty + \Vert\overline{\bp}_i^{\odot\frac{1}{2}}\Vert_\infty  \Vert\bb_i\Vert_\infty \Vert\bp_i^{\odot-1}\Vert_\infty +\\
    &\quad C^2\sqrt{\frac{F}{T}} \left[ \frac{1}{K} \sum_{k=1}^K \Vert\bq_{i,k}\Vert_\infty \Vert\bp_{i,k}^{\odot-\frac{1}{2}}\Vert_\infty + \Vert\overline{\bp}_i^{\odot\frac{1}{2}}\Vert_\infty \Vert\bq_i\Vert_\infty \Vert\bp_i^{\odot-1}\Vert_\infty \right] \max\left(\sqrt{\frac{\log\left(\frac{2}{\delta}\right)}{c}},  \sqrt{\frac{F}{T}}\frac{\log\left(\frac{2}{\delta}\right)}{c}\right).
\end{align*}

